mmFHE: mmWave Sensing with End-to-End Fully Homomorphic Encryption

We present mmFHE, the first system that executes the entire cloud-side mmWave sensing pipeline including the DSP and ML inference under fully homomorphic encryption (FHE). mmFHE encrypts range profiles on an edge device after lightweight plaintext preprocessing and executes the entire mmWave signal-processing and ML inference pipeline homomorphically on a semi-honest cloud that operates exclusively on ciphertexts. At the core of mmFHE is a library of seven composable, data-oblivious FHE kernels that replace standard DSP routines with fixed arithmetic circuits for different application-specific pipelines. We demonstrate this approach on two representative tasks: vital-sign monitoring and gesture recognition. We formally prove two cryptographic guarantees for any pipeline assembled from this library: input privacy and data obliviousness. These guarantees effectively neutralize various supervised and unsupervised privacy attacks on raw data, including re-identification and data-dependent privacy leakage. Evaluation on three public radar datasets shows that encryption introduces negligible error versus the plaintext pipeline, with 84.5% gesture accuracy (vs. 84.7%). End-to-end cloud GPU latency is 1.21 s per 10 s vital-sign window and 5.76 s per 3 s gesture window. These results establish the initial feasibility of end-to-end mmWave sensing under FHE on commodity hardware.

==> figures/architecture_diagram.tex <==
a


==> sections/3-preliminaries.tex <==
\section{mmFHE}
\label{sec:background}

\subsection{Approach}

\name{} encrypts the entire radar DSP pipeline under Cheon-Kim-Kim-Song (CKKS) homomorphic encryption, which runs on \rev{semi-honest} cloud server while providing input security and data obliviousness.

% Both chains require spectral transforms, non-linear detection, and data-dependent operations that must be reformulated for encrypted computation (\S\ref{sec:system_design}).

\input{sections/4-threat-model}

\subsection{Homomorphic Encryption Primer}
\label{subsec:he_primer}

Fully homomorphic encryption (FHE) allows a server to compute on
encrypted data without ever seeing the plaintext. The client encrypts
its input, sends the ciphertext to the server, and the server returns
an encrypted result that only the client can decrypt. No secret key
material leaves the client. We use the Cheon, Kim, Kim, and Song (CKKS) FHE scheme~\cite{cheon2017homomorphic}, which is designed for
\textit{approximate} arithmetic on real and complex numbers, suitable for radar signal processing. Unlike exact-integer schemes
(BFV/BGV~\cite{fan2012somewhat}) or Boolean-circuit schemes
(TFHE~\cite{chillotti2020tfhe}), CKKS treats encryption noise as
part of the numerical error, analogous to floating-point rounding.

\noindent\textbf{Security.}
CKKS security relies on the Ring Learning with Errors (RLWE)
problem~\cite{lyubashevsky2013ideal}, a lattice-based hardness
assumption believed to resist both classical and quantum attacks.
A ciphertext in CKKS is a pair of polynomials in the ring $\mathbb{Z}_Q[X]/(X^N+1)$, simply meaning polynomials with coefficients modulo $Q$ where we treat $X^N$ as $-1$. So every element is just $N$ coefficients and multiplication wraps around with a sign flip. CKKS also provides a public key ($pk$), and a secret key ($sk$). Given only the ciphertext and $pk$, no efficient adversary can determine which of two messages was encrypted (a property known as IND-CPA, or indistinguishability under chosen-plaintext attack~\cite{katz2020introduction}). The security level depends on
two parameters: the polynomial degree $N$ (larger $N$ is stronger)
and the coefficient modulus $Q$ (larger $Q$ is weaker). We follow the
HE Standard~\cite{HomomorphicEncryptionSecurityStandard} to achieve
$\geq 128$-bit security, comparable to AES-128 \cite{}.

\noindent\textbf{Encoding and SIMD Batching.}
A key efficiency feature of CKKS is that a single ciphertext packs up
to $N/2$ real values into parallel \textit{slots}. All arithmetic
applies slot-wise, so one ciphertext operation processes $N/2$ values
simultaneously. For example, with $N{=}32768$, a single encrypted add
or multiply acts on 16{,}384 values at once. This single instruction, multiple data (SIMD) batching is what makes encrypted radar DSP practical: an entire range profile or Doppler spectrum fits in one ciphertext.

\noindent\textbf{Depth Budget: The Central Constraint.}
Every CKKS ciphertext carries a finite \textit{multiplicative depth}
budget $L$. Each multiplication between two ciphertexts consumes one
level; after $L$ multiplications, the ciphertext can no longer be
used. Addition, by contrast, is free and does not consume any depth.
This budget is the primary design constraint for encrypted signal
processing: the entire DSP pipeline must be expressed as a circuit
with at most $L$ sequential multiplications. Deeper circuits require
either a larger $N$ (more memory and compute) or
\textit{bootstrapping}---a costly operation that refreshes the depth
budget. \name{} pipelines are designed to fit within their depth
budgets without bootstrapping.

\noindent\textbf{Three Primitive Operations.}
All encrypted computation is built from three operations:\\
% \begin{itemize}
    \noindent \textit{Addition:} $\mathsf{Enc}(\mathbf{a}) + \mathsf{Enc}(\mathbf{b}) = \mathsf{Enc}(\mathbf{a}+\mathbf{b})$. Slot-wise vector addition. Free in depth, negligible cost.\\
    \noindent \textit{Multiplication:} $\mathsf{Enc}(\mathbf{a}) \cdot \mathsf{Enc}(\mathbf{b}) = \mathsf{Enc}(\mathbf{a} \odot \mathbf{b})$. Slot-wise element-wise multiplication. Consumes one depth level.\\
    \noindent \textit{Rotation:} $\mathsf{Rot}(\mathsf{Enc}(\mathbf{a}), k)$ cyclically shifts the slot vector by $k$ positions. Free in depth but requires pre-generated \textit{Galois keys} (one per rotation amount). Rotations enable cross-slot operations such as inner products and convolutions.\\
% \end{itemize}

\noindent These three primitives are sufficient for addition,
scaling, polynomial evaluation, and matrix-vector products. However,
non-linear functions such as $\arg\max$, comparison, and
$\arctan$ have no direct encrypted counterpart. They must be
\textit{approximated} as polynomial circuits subject to the depth
budget $L$. 
% This constraint drives every design choice in
% \S\ref{sec:system_design}: replacing hard detection with soft
% polynomial attention, expressing FFTs as matrix multiplies, and using
% square activations instead of ReLU.

Table~\ref{tab:ckks_params} summarizes the CKKS parameters used in
\name{} pipelines.

\begin{table}[t]
  \centering
  \caption{CKKS parameters for \name{} pipelines. 
  % Both configurations achieve $\geq 128$-bit security per the HE Standard~\cite{HomomorphicEncryptionSecurityStandard}.
  }
  \label{tab:ckks_params}
  \footnotesize
  \begin{tabular}{@{}lcc@{}}
    \toprule
    \textbf{Parameter} & \textbf{Vital Signs} & \textbf{Gesture} \\
    \midrule
    Ring dimension $N$ & \placeholder & $2^{15}$ (32768) \\
    Slots ($N/2$) & \placeholder & 16384 \\
    Mult.\ depth $L$ & \placeholder & 11 \\
    Scaling mod.\ size & 40 bits & 50 bits \\
    First/last mod.\ size & 60 bits & 60 bits \\
    Scaling technique & \multicolumn{2}{c}{FLEXIBLEAUTO} \\
    Security level & $\geq 128$ bits & $\geq 128$ bits \\
    Bootstrapping & No & No \\
    \bottomrule
  \end{tabular}
\end{table}


==> sections/4-threat-model.tex <==
\subsection{Threat Model}
\label{sec:threat_model}

[from raja: what scenario - what are the attacker capable of - what are protecting from - what we are not protectig from] only these 4 things


Consider a mmWave presence detector deployed for smart lighting. It needs only the magnitude of complex range profiles to detect occupancy, not the phase. But providing the raw IQ stream for magnitude-based detection simultaneously and unavoidably discloses the phase, and phase encodes heartbeat, respiration, gait, and speech. This coupling is not incidental: we show it is mathematically unavoidable, and its consequences are measurable. On a public 60\,GHz gesture dataset~\cite{zenodo_gesture}, a random-forest classifier achieves 99.9\% user re-identification accuracy from raw IQ features within a session, and 78.6\% across physically different gesture types. On a 77\,GHz vital-sign dataset of 50 children~\cite{children_dataset} intended solely for HR/RR tracking, the same classifier infers age group at 76\% accuracy (vs.\ 33\% chance). Neither inference was an intended use of the data. (Want to motivate with a concreate threat as above)


Consider the following question: can a client delegate computation on raw sensor streams without exposing sensitive micro-motion information embedded in those streams? We show that, for plaintext protocols, the answer is no.

\noindent\textbf{The Inseparability of Detection and Micro-Motion.}
\label{subsec:inseparability}
A fundamental premise of \name{} is that sharing raw radar data for one purpose (e.g., presence detection) inherently exposes the full micro-motion signature of every observed target. We formalize this as the \textit{Inseparability Property} of coherent radar streams.

\begin{theorem}[Inseparability Property of Coherent Radar Streams]
\label{thm:biometric_inseparability}
Let $\{\mathbf{z}[r, t]\}_{t=1}^{F}$ be a plaintext FMCW range-profile stream with carrier wavelength $\lambda$, slow-time sampling rate $f_s \geq 2 f_{\mu}$ (where $f_{\mu}$ is the highest micro-motion frequency of interest), and observation duration $F/f_s \geq T_{\min}$. Then any protocol that grants a semi-honest server plaintext access to this stream for energy-based target detection $r$, necessarily leaks sufficient information to reconstruct the target's radial micro-displacement signal at all frequencies up to $f_{\mu}$.
\end{theorem}

\begin{proof}
    Refer to Appendix \ref{sec:app_A}.
\end{proof}

% \begin{proof}
% \noindent\textit{Algebraic inseparability:}
% Energy-based detection requires computing $E_k[t] = |\mathbf{z}_k[t]|^2$ from plaintext range-bin values $\mathbf{z}_k[t] \in \mathbb{C}$. To evaluate this, the server \underline{\textit{must}} receive the complex samples $\mathbf{z}_k[t]$.
% % (or equivalent raw ADC inputs $\mathbf{x}[t]$ from which $z_k[t]$ is recoverable via the invertible DFT: $\mathbf{z}[t] = \mathbf{F}\mathbf{x}[t]$). Each $z_k[t]$ decomposes uniquely in polar form as $(|z_k[t]|,\; \phi_k[t])$. 
% Providing $\mathbf{z}_k[t]$ for magnitude-based detection therefore simultaneously and unavoidably discloses the phase $\phi_k[t]$. A semi-honest server logs all inputs, making this leakage immediate and irreversible.

% \noindent\textit{Phase--displacement coupling:}
% By the FMCW radar equation (\S\ref{subsec:fmcw_primer}), small radial displacements $\Delta d_k[t]$ of the target at range bin $k$ induce phase shifts $\Delta \varphi_k[t] = {4\pi \Delta d_k[t]}/{\lambda}$. This mapping is linear and invertible, so the adversary recovers $\Delta d_k[t]$ from the disclosed phase sequence.

% \noindent\textit{Nyquist sufficiency:}
% The adversary now holds $F$ samples of $\Delta d_k[t]$ at rate $f_s \geq 2 f_{\mu}$ over a duration $F/f_s \geq T_{\min}$. By the Shannon--Nyquist theorem, this is sufficient to reconstruct the continuous-time micro-displacement signal and resolve its spectral components at all frequencies up to $f_{\mu}$.
% \end{proof}


The micro-displacement signal $\Delta d_r(t)$ encodes any physical phenomenon that produces sub-wavelength radial motion. Examples include: vital signs such as respiration (${\sim}0.3$\,Hz) and heartbeat (${\sim}1$--$2$\,Hz), gait micro-Doppler (${\sim}5$\,Hz) enabling re-identification~\cite{vandersmissen2018gait}, hand tremor patterns indicative of neurological conditions, and even speech recovery from vocal-cord vibrations ($f_{\mu} \sim 300$\,Hz)~\cite{wang2022mmspy}. The inseparability property implies that \emph{any} protocol granting plaintext access for detection simultaneously enables all of these inferences to a semi-honest cloud server.

% \noindent
% We note that secret-sharing or multi-party computation (MPC) schemes could in principle compute on shares without exposing the $z_k[t]$ stream, but they require non-colluding servers and incur communication overheads that complicate resource-constrained IoT deployments, and hence are outside the scope of this work.

\noindent\textbf{Adversary Model.}
We adopt the \textit{semi-honest} (honest-but-curious) adversary model: the cloud faithfully executes the agreed-upon protocol but may analyze everything it observes: inputs, intermediate values, and execution behavior; to infer sensitive information. In this setting, two fundamental sources of information leakage arise:
\begin{itemize}
    \item \textbf{The raw data:} By the inseparability property, plaintext radar samples $\{\mathbf{z}[r, t]\}_{t=1}^{F}$ expose the full micro-displacement spectrum. A semi-honest server can extract unauthorized information far beyond the scope of the authorized application.
    \item \textbf{The DSP algorithms:} Standard radar signal processing routines (e.g., CFAR detection, Kalman filtering) contain inherently \textit{data-dependent} control flow: they branch, prune, or allocate resources based on input values. Even without reading data content, a semi-honest server can infer target presence and location from memory access patterns, instruction traces, and timing variations.
\end{itemize}
\noindent While more sophisticated attacks may combine these two channels (e.g., correlating partial content leakage with execution timing), they fundamentally rely on at least one channel being compromised. We therefore focus on neutralizing both channels independently.
% , which by construction eliminates combined attacks as well. 
% We note that the semi-honest model does not address integrity violations (e.g., a malicious server returning fabricated results); verifiable computation extensions are discussed in future works.

\noindent\textbf{Capabilities \& Constraints.}
The adversary is probabilistic polynomial-time (PPT) and cannot break the Ring-LWE assumption underlying CKKS (\S\ref{subsec:he_primer}). It has full visibility into server-side memory, execution traces, and all ciphertexts and public parameters received from the client.

\noindent\textbf{Our Solution.}
To neutralize both leakage channels, we require a mechanism that provides (i)~cryptographic data secrecy during computation and (ii)~data-oblivious execution. 
% Differential privacy destroys the sub-millimeter phase precision vital signs demand~\cite{sun2024sok_wireless}; trusted execution environments (SGX, TrustZone) suffer from microarchitectural side channels~\cite{kocher2019spectre,lipp2018meltdown,murdock2020plundervolt} and do not guarantee obliviousness; multi-party computation incurs prohibitive communication for streaming radar; and federated learning protects training data, not inference-time sensor streams.
CKKS FHE is the only mechanism that satisfies both requirements without hardware trust assumptions. Under our proposed \name{}, the client encrypts the range-profile stream and the server evaluates the entire DSP pipeline homomorphically on $\mathsf{Enc}(\{\mathbf{z}[t]\}_{t=1}^{F})$, never observing any plaintext value. The server \emph{does} know the circuit being evaluated (e.g., DSP algorithms); the security guarantee relies on semantic security (IND-CPA) under the Ring-LWE assumption. By further designing all server-side kernels as fixed arithmetic circuits (\S\ref{sec:system_design}), we ensure the execution trace is independent of the input data, closing the side-channel as well. We provide formal proofs of both properties in \S\ref{sec:security}. Thus, \name{} breaks the inseparability of Theorem~\ref{thm:biometric_inseparability} via encryption. \textit{If the the underlying conditions are met with $f_s, f_\mu, F, T_{\text{min}}$; the server evaluates detection and tracking circuits without learning anything about the phase.}
% and the client selectively decrypts only the outputs its application requires---presence for a lighting service, vital signs for health monitoring---withholding everything else.

\noindent\textbf{Security Goals.}
Against this adversary, \name{} provides two complementary guarantees: (1)~\textit{Input Privacy}: the cloud learns nothing about the content of encrypted sensor streams (Theorem~\ref{thm:input_privacy}); and (2)~\textit{Data Obliviousness}: the cloud's execution trace is independent of the sensor data (Proposition~\ref{thm:data_oblivious}). 
% Together, these defeat content-based attacks (Scenario~1) and side-channel attacks (Scenario~2), respectively.


\noindent\textbf{Trust boundary.}
The \textit{client} (edge radar device) is trusted: it holds the secret key, performs encryption and decryption, enforces disclosure policies, performs Range FFT and executes clutter removal locally before uploading ciphertexts. The \textit{cloud} server is \rev{semi-honest}: it receives only ciphertexts and public evaluation keys, and executes the encrypted DSP and ML inference circuit. In this work, 
% We do not model other physical side-channel attacks on the client (e.g., power analysis of the sensor) or network-level traffic analysis as our 
we primarily focus on protecting data-in-transit and data-in-use at the cloud; so other physical side-channel attacks are out of scope. However, the number and size of ciphertexts are fixed by public configuration and independent of data content, limiting metadata leakage to session-level information (\S\ref{subsec:leakage}).

\noindent\textbf{Illustrative scenarios.}
\label{subsec:attack_scenarios}
To ground the above threats concretely:
\textit{(1)~Unauthorized micro-motion profiling.}
A ``Smart Lighting'' app requires only presence detection, yet in a plaintext protocol the cloud receives $\{\mathbf{z}[r,t]\}_{t=1}^{F}$ and can extract phase-derived vital signs, gait signatures, or speech by the inseparability property (Theorem~\ref{thm:biometric_inseparability}).
Under \name{}, the server operates on ciphertexts; the client decrypts only presence-level outputs.
\textit{(2)~Trajectory inference via access patterns.}
Standard CFAR detection branches on $|\mathbf{z}_k|^2 > \tau$, leaking which range bins contain targets through memory access traces---even if data values are encrypted.
\name{} evaluates all bins uniformly via fixed arithmetic circuits, making the execution trace independent of the scene.

\noindent\textbf{Existing FHE Solutions are Insufficient.}
% Existing FHE-based radar systems encrypt only the classification
% stage, leaving the upstream DSP pipeline in plaintext.
RPRS~\cite{wu2025rprs},
the most directly comparable system, encrypts only the final FC
classifier: the entire radar DSP chain: range FFT, Doppler FFT, CFAR
detection, and filtering executes in plaintext on local server before
features are encrypted and sent to the cloud. This means all
intermediate representations (range-Doppler maps, point clouds,
detected peaks) remain exposed (by
Theorem~\ref{thm:biometric_inseparability}).
% , these plaintext
% intermediates carry the full micro-displacement spectrum: an
% honest-but-curious local server running RPRS-style plaintext DSP can extract vital signs, gait signatures, or speech from the very features it
% computes. 
Cruicially, encrypting only the classifier protects the model, not the
user. \name{} closes this gap by encrypting the \textit{entire}
pipeline from raw range profiles through detection, feature
extraction, and classification, ensuring no intermediate
representation is ever exposed in plaintext on the server.




==> sections/5-mmFHE_March12_arxived.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section: System Design
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{System Design}
\label{sec:system_design}
\label{sec:pipeline}
% The vital signs pipeline requires two lightweight decryptions 
% (target-bin index and
% HR/RR BPM values); the classification pipeline requires a single
% logit-vector decryption. All decryptions occur on the trusted client.

%-------------------------------------------------------------------
\subsubsection{Overview}
\label{subsec:architecture}
\begin{figure*}[t]
    \centering
    \resizebox{0.95\textwidth}{!}{\input{figures/architecture_diagram.tex}}
    \caption{\name{} architecture. The client performs lightweight
    pre-processing and encryption; the cloud executes the full
    encrypted DSP and inference pipeline using composable kernels; the
    client decrypts only authorized scalar outputs. Two application
    compositions are shown: vital signs (left path) and ML inference
    (right path). The secret key $sk$ is shared only between the
    trusted client endpoints.}
    \label{fig:arch}
\end{figure*}

\name{} breaks the inseparability theorem (Theorem~\ref{thm:biometric_inseparability}) by
encrypting range profiles on the client and executing the entire
signal-processing and inference chain over ciphertexts on the cloud.
The cloud never observes any plaintext value, and every kernel runs as
a fixed arithmetic circuit whose execution trace is independent of the
input data; closing both the content leakage and side-channel leakage
identified in \S\ref{sec:threat_model}. \name{} provides a library of seven FHE-compatible DSP kernels that compose into complete application pipelines. The cloud chains these kernels over ciphertexts, and the trusted client decrypts only authorized scalar outputs. Figure~\ref{fig:arch} summarizes the system architecture:

\begin{enumerate}
  \item Trusted \textbf{Client} does the following:
  
  \begin{itemize}
      \item Pre-encrypt stage: after receiving Range-FFT from mmWave sensor, removes clutter and normalizes data.
      \item Encryption stage: generates CKKS keys $(pk, sk, gk)$. The secret key $sk$ never leaves the trusted client device(s). Encrypts normalized data using $pk$ before packing and sending the ciphertext with the $gk$ to the cloud. 
      \item Decryption and output stage: after receiving encrypted results from the cloud, client decrypts using $sk$ and authorized outputs such as: HR/RR waveforms, HR/RR BPM values, target-bin index, or the logit vector for
        classification.
  \end{itemize}


  \item Semi-honest \textbf{Cloud} receives ciphertext and $gk$ from the client. Selects and chains kernels from the \name{} library
        according to the target application. Each kernel is a fixed
        arithmetic circuit ($gk$ is required for some kernels); performing on the ciphertext. Cloud sends encrypted result back to the client. The cloud never observes plaintext values.
        % Concrete pipeline compositions are described in
        % \S\ref{subsec:pipeline_vitals} and
        % \S\ref{subsec:pipeline_gesture}.
\end{enumerate}

%-------------------------------------------------------------------
\subsubsection{Pre-Cloud Client-Side Algorithms}
\label{subsec:client_preprocessing}

Let the raw input be per-antenna complex range profiles
$\mathbf{z}[t] =z_{a}[r]\in \mathbb{C}^{R \times A}$ for frames
$t=1,\ldots,F$, where $R$ is the number of range bins and $A$ is
the number of antenna elements.

\noindent\textbf{Range FFT and Preprocessing.}
The client computes the range FFT (Eq.~\ref{eq:range_fft}) locally
for each antenna and chirp, selects $R$ range bins, and applies
clutter removal via mean subtraction
$\tilde{\mathbf{z}}[t] = \mathbf{z}[t] -
\frac{1}{F}\sum_{l}\mathbf{z}[l] $. Values are then scaled to a
numerically stable range: frame-local normalization for vital signs
(the scalar cancels in differential phase), batch-global for
gestures. 
% The lowest range bins are zeroed to suppress near-field
% leakage. 
% This is the only FFT in the pipeline; all subsequent
% spectral operations are reformulated as matrix-vector products
% executable under CKKS.

\noindent\textbf{Encryption and Packing.}
 CKKS operates on real-valued slot vectors, complex radar data $\tilde{\mathbf{z}}[t] = \mathbf{v}^{(\mathrm{re})}+j\cdot\mathbf{v}^{(\mathrm{im})}$
is split into separate real and imaginary ciphertexts:
$\hat{\mathbf{v}}^{(\mathrm{re})} =
\mathsf{Enc}_{pk}(\mathbf{v}^{(\mathrm{re})})$,
$\hat{\mathbf{v}}^{(\mathrm{im})} =
\mathsf{Enc}_{pk}(\mathbf{v}^{(\mathrm{im})})$, where
$\{\mathbf{v}^{(\mathrm{re})}, \mathbf{v}^{(\mathrm{im})}\} \in
\mathbb{R}^{N/2}$ is an encrypted frame. The packing strategy differs by pipeline:
\begin{itemize}
  \item \emph{Vital signs:} each frame is packed across $R$ range bins
        into the first $R$ slots. 
        % \item Energy accumulation happens across
        % per-frame ciphertexts via homomorphic addition.
  \item \emph{Doppler pipelines (e.g., dynamic classification):}
        per-frame data from $A$ antennas $\times$ $R$ range bins
        $\times$ $D$ chirps is interleaved using
        $\text{slot}[a \cdot RD + r \cdot D + c]$, yielding $ARD$
        active slots out of $N/2$ total. This layout places each
        antenna-range group's $D$ chirps in contiguous slots, enabling
        the block-diagonal Doppler DFT (Kernel~3) to operate via
        slot rotations within each $D$-element block.
\end{itemize}

%-------------------------------------------------------------------
\subsubsection{Cloud-Side Algorithms}
\label{subsec:cloud_processing}

The cloud receives ciphertexts and public parameters only. All \name{}
kernels are data-oblivious: they execute the same sequence of
additions, multiplications, and rotations regardless of the
encrypted input, ensuring the execution trace leaks no information
about the radar scene (formalized in
Theorem~\ref{thm:data_oblivious}).

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\noindent\textbf{Kernel 1: Energy Integration}
\label{subsec:energy}
Computes per-bin signal power $|\tilde{z}_r[t]|^2$.  For each range bin $r$, the cloud computes:
\begin{equation}
  E_r \;=\; \sum_{t=1}^{F}
  \Bigl(\mathrm{Re}(\tilde{z}_r[t])^2 + \mathrm{Im}(\tilde{z}_r[t])^2\Bigr).
  \label{eq:energy}
\end{equation}

$E_r $ is computed on a fresh ciphertext (depth~1) and accumulated via homomorphic addition across frames (depth-free). The output is a single packed ciphertext
containing all $R$ bin energies. \textbf{Depth consumed: 1.}
\textit{Used in:} vital signs (target detection), dynamic
classification ($|z|^2$ power spectrum).

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\noindent\textbf{Kernel 2: Soft Power Attention}
\label{subsec:soft_argmax}
Standard radar CFAR thresholding or hard argmax replacement in \name{}. A branch-free polynomial attention mechanism that processes every bin uniformly. Given an energy profile $E_r$, \name{} computes power-weighted statistics:
\begin{align}
  w_r &= E_r^{\gamma}, \label{eq:soft_power_weight} \\
  N = \sum_{r=0}^{R-1} r\,w_r,
  &\qquad 
  D = \sum_{r=0}^{R-1} w_r,
  \label{eq:soft_argmax_stats}
\end{align}
where the sharpening exponent $\gamma$ controls the concentration of weight on dominant bins. Analogous to a Boltzmann distribution with inverse temperature $\beta = \gamma$: at $\gamma{=}1$, the weighted statistics reduce to an energy centroid; as $\gamma \to \infty$, weight concentrates entirely on the maximum-energy bin, recovering hard argmax. Enables computing first-moment estimate $\hat{r} = N/D$.
$ w_r $ is computed via sequential square operations, each consuming depth~1; higher $\gamma$ gives sharper selection at the cost of more depth.

In our experiments, $\gamma{=}2$ is sufficient for energy profiles,: a
single ciphertext-ciphertext squaring ($E_r^2$) at depth~1. 
% The cloud returns encrypted $\mathsf{Enc}(N)$ and $\mathsf{Enc}(D)$; the client decrypts and divides to recover the soft target-bin estimate $\hat{r} = N/D$. 
While $\gamma{=}4$ provides sharper selection for range-Doppler power profiles, when operating over the Doppler dimension:
\begin{equation}
  s[d] = \left(\sum_{a=0}^{A-1}\sum_{r=0}^{R-1} |{\mathbf{Z}}_{a}[r,d]|^2\right)^{\!\gamma}
  \label{eq:gesture_soft_power}
\end{equation}
The summation across antennas and range bins uses rotations and additions only (zero depth). The power $\gamma{=}4$ is computed as two sequential square operations (depth~2). The resulting weights are replicated back to all $ARD$ slots via reverse rotations and additions (zero depth), then multiplied element-wise with the power spectrum to produce weighted features (depth~1). \textbf{Depth consumed:} 1 to 3.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\noindent\textbf{Kernel 3: DFT via Block-Diagonal Matmul}
\label{subsec:doppler_dft}
In a standard FFT, each butterfly stage consumes one multiplicative depth level.
% : prohibitive for the small block sizes in our pipeline ($D{=}8$). 
To optimize, we instead express the windowed, shifted DFT
as a plaintext matrix-vector multiply, which decomposes into
additions, multiplications by plaintext constants, and rotations while consuming only a single depth level.  A windowed DFT kernel ($D \times D$):
\begin{equation}
  \mathbf{W}=W_{d,n} = w[n] \cdot e^{-j\frac{2\pi}{D}\sigma(d) \cdot n},
  \quad d,n \in [D]
  \label{eq:dft_kernel}
\end{equation}
where $w[n]$ is the Hanning window and $\sigma$ is the
\texttt{fftshift} permutation ($\sigma(d) = (d+D/2) \bmod D$).
Splitting into real and imaginary parts $\mathbf{C} = \mathbf{W}^{(\mathrm{re})}$,
$\mathbf{S} = \mathbf{W}^{(\mathrm{im})}$, and tiling block-diagonally
$AR$ times to match the slot layout:
\begin{align}
  &\hat{\mathbf{d}}^{(\mathrm{re})} =
    \tilde{\mathbf{C}} \cdot \hat{\mathbf{v}}^{(\mathrm{re})}
    - \tilde{\mathbf{S}} \cdot \hat{\mathbf{v}}^{(\mathrm{im})},
  \label{eq:dft_re} \\
  &\hat{\mathbf{d}}^{(\mathrm{im})} =
    \tilde{\mathbf{S}} \cdot \hat{\mathbf{v}}^{(\mathrm{re})}
    + \tilde{\mathbf{C}} \cdot \hat{\mathbf{v}}^{(\mathrm{im})},
  \label{eq:dft_im}
\end{align}
where $\tilde{\mathbf{C}} = \mathbf{I}_{AR} \otimes \mathbf{C}$ and $\tilde{\mathbf{S}} = \mathbf{I}_{AR} \otimes \mathbf{S}$ are
the block-diagonal replications.

\noindent\textbf{BSGS optimization.}
Each matrix-vector product is implemented via the Halevi-Shoup
diagonal method~\cite{halevi2014algorithms} with baby-step/giant-step
(BSGS) decomposition. The standard diagonal method decomposes
$\mathbf{A}\mathbf{x} = \sum_i \mathrm{diag}_i(\mathbf{A}) \odot
\mathrm{Rot}(\mathbf{x}, i)$, requiring one rotation per non-zero
diagonal. BSGS splits the index $i = g \cdot b + s$ into giant steps
$g$ and baby steps $s$, reducing the total rotation count from $d$ to
$\lceil\sqrt{d}\,\rceil + \lceil d/\sqrt{d}\,\rceil \approx
2\sqrt{d}$. 
% Because all $AR$ blocks are identical, the
% block-diagonal structure yields only ${\sim}15$ unique diagonals
% (instead of $ARD$), requiring ${\sim}112$ rotation keys.
\textbf{Depth consumed: 1}
(plaintext-ciphertext matmul).
\textit{Used in:} dynamic classification.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\noindent\textbf{Kernel 4: Soft I/Q Extraction of Highest-Energy Bin}
\label{subsec:phase}
For each frame $t$, the cloud computes a per-frame energy mask which concentrates on the highest-energy range bin without data-dependent selection and extracts soft-weighted I/Q scalars:
\begin{align}
  m_r[t] &= [\mathrm{Re}(\tilde{\mathbf{z}}_r[t])^2 + \mathrm{Im}(\tilde{\mathbf{z}}_r[t])^2]^{P_\phi},
  \label{eq:phase_mask} \\
  I[t] &= \sum_{r=0}^{R-1} m_r[t] \cdot \mathrm{Re}(\tilde{\mathbf{z}}_r[t]),
  \nonumber \\
  Q[t] &= \sum_{r=0}^{R-1} m_r[t] \cdot \mathrm{Im}(\tilde{\mathbf{z}}_r[t]).
  \label{eq:phase_iq}
\end{align}
Each output $(\mathbf{I}, \mathbf{Q})=(I[t], Q[t])$ remains encrypted and feeds directly into relevant subsequent kernels without intermediate decryption. From our experiments, $P_\phi=2$ is sufficient. \textbf{Depth consumed: 3}.
\textit{Used in:} vital signs.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\noindent\textbf{Kernel 5: FIR Filtering}
\label{subsec:fir}
FIR (finite impulse response) filters are pure
feedforward: each output is a weighted sum of a fixed window of
inputs, expressible as a single matrix-vector multiply:
\begin{equation}
  \mathbf{I}^{(b)}_{f} = \mathbf{T}^{(b)} \mathbf{I},
  \qquad
  \mathbf{Q}^{(b)}_{f} = \mathbf{T}^{(b)} \mathbf{Q},
  \label{eq:fir_iq}
\end{equation}
where $\mathbf{T}^{(b)}$ is the Toeplitz matrix for pass-band $b$.

\noindent\textbf{Alternate Implementation.}
FIR filtering can also be realized via weighted accumulation over slot rotations: $y[n] = \sum_k h[k] \cdot \mathrm{Rot}(\mathbf{x}, k)$, where $h[k]$ are the plaintext filter taps. \textbf{Depth consumed: 1}.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\noindent\textbf{Kernel 6: Notch Mask}
\label{subsec:notch}
For static clutter removal in Range-Doppler under FHE, we present a fixed binary plaintext mask:
\begin{equation}
  m[d] = \begin{cases}
    0, & d \in [\lfloor D/2 \rfloor, \lceil D/2 \rceil) \\
    1, & \text{otherwise}
  \end{cases}
  \label{eq:notch_mask}
\end{equation}
The mask is a
public constant and does not depend on the input. \textbf{Depth consumed: 1}.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\noindent\textbf{Kernel 7: Differential Phase Extraction via Taylor Series Approximation}
\label{subsec:taylor_arctan}
We replace the $\arctan(Q/I)$ with a low-order Taylor expansion that operates directly on consecutive filtered samples. Given
\begin{align}
  y[t] &= Q_f[t]\,I_f[t{-}1] - I_f[t]\,\mathbf{Q}_f[t{-}1],
  \nonumber \\
  x[t] &= I_f[t]\,I_f[t{-}1] + Q_f[t]\,\mathbf{Q}_f[t{-}1],
  \nonumber \\
  \Delta\phi[t] &\approx y[t]\,x[t]^2 - \tfrac{1}{3}\,y[t]^3,
  \label{eq:taylor_arctan}
\end{align}
a third-order Taylor expansion of $\arctan(y/x)$ requiring three
ciphertext-ciphertext multiplicative depth levels. For low-SNR
scenarios where $|\Delta\phi| \ll 1$, a first-order approximation
$\Delta\phi \approx y$ suffices, trading accuracy for a
shallower circuit. \textbf{Depth consumed: 3}.

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\noindent\textbf{Encrypted ML Inference}
\label{subsec:mlp}
Following standard practice for encrypted neural
inference~\cite{wu2025rprs,hear2022}, we use a fully connected (FC) network with
square activations ($\sigma(x) = x^2$). The optimized weights $\{\mathbf{W}^{(\ell)},
\mathbf{b}^{(\ell)}\}$ are shipped to the cloud as public
plaintext parameters.  For each layer $\ell = 1, \ldots, L$:
\begin{equation}
  \mathbf{h}^{(\ell)} =
  \begin{cases}
    \bigl(\mathbf{W}^{(\ell)} \mathbf{h}^{(\ell-1)} +
    \mathbf{b}^{(\ell)}\bigr)^{\circ 2}
    & \ell < L,\\[4pt]
    \mathbf{W}^{(L)} \mathbf{h}^{(L-1)} + \mathbf{b}^{(L)}
    & \ell = L,
  \end{cases}
  \label{eq:mlp_forward}
\end{equation}
where $(\cdot)^{\circ 2}$ denotes element-wise squaring. 

\noindent\textbf{Weight folding.}
The soft power normalization factor $s^\gamma / F$ and the column
permutation that reorders the encrypted slot layout to match the
training feature order are both folded into
$\mathbf{W}^{(1)}$ at setup time---plaintext operations on the weight
matrix at zero depth cost. Where $s = R · A · (\sum_n w[n])^2$ is the expected spectral energy scale. \textbf{Depth consumed: 2L -1.}

%-------------------------------------------------------------------
\subsubsection{Post-Cloud Client-Side Result Recovery}
\label{subsec:result_recovery}

After cloud execution, the client selectively decrypts only the
outputs authorized for the target application. The client decrypts the returned ciphertexts results using $sk$: $$\mathsf{Dec}_{sk}(\mathsf{Enc}_{pk}(\text{\textit{result}}))$$ for \textit{result $\in$ $\{$HR, heart waveform, RR, respiration waveform, target bin N/D, ML logits$\}$}. No post-processing beyond scalar division and plaintext argmax are required.

% \medskip\noindent\textbf{Selective disclosure.} The client holds the
% sole decryption key and chooses which outputs to decrypt. A
% vital-sign monitor decrypts only $\hat{r}$ and the HR/RR BPM
% scalars; a classification client decrypts only the logit vector. All
% other information---phase signatures, Doppler spectra, intermediate
% features---remains cryptographically sealed in ciphertexts the client
% never decrypts.

%-------------------------------------------------------------------

%-------------------------------------------------------------------
\subsubsection{Example Application Pipelines}
\label{subsec:pipeline_vitals}
Two examples are provided below:

\noindent\textbf{Encrypted Vital Signs}
The vital signs pipeline chains
K1$\to  \allowbreak$K2$\to$K4$\to$K5$\to$K7 plus three pipeline-specific stages
(partial DFT, power spectrum, spectral soft-argmax). Energy
integration and soft attention (K1--K2) localize the target bin
(first decrypt: $\hat{r}=N/D$). Phase extraction (K4) and FIR
filtering (K5) produce bandpassed I/Q traces for respiration
(0.1--0.6\,Hz) and heart rate (0.8--2.5\,Hz). Taylor arctan (K7)
recovers differential phase, followed by a narrowband DFT over $K$
passband bins, power spectrum $|X[k]|^2$, spectral sharpening, and
weighted frequency average (second decrypt: HR/RR in BPM). Total
circuit depth: 11 (third-order Taylor) or 9 (first-order).
Optionally, the encrypted phase waveform (after K5) can be returned
for client-side visualization. See Table~\ref{tab:depth} for the
full depth accounting.

%-------------------------------------------------------------------
\noindent\textbf{Encrypted Dynamic Radar Classification}
\label{subsec:pipeline_gesture}

The classification pipeline processes $F$ frames, accumulating
weighted features before a single FC pass. Per frame: Doppler DFT
(K3) produces the encrypted range-Doppler spectrum; squared magnitude
(K1) and soft power attention with notch mask (K2+K6, $\gamma{=}4$)
extract weighted features; features accumulate across frames via
addition (free). The accumulated vector passes through the encrypted
FC network (\S\ref{subsec:mlp}):
FC$_1$+$x^2$ $\to$ FC$_2$+$x^2$ $\to$ FC$_3$ (logits).
Total circuit depth: 11. The client decrypts the 5-class logit vector
and applies plaintext argmax. The architecture generalizes to any
classification task over temporal radar signatures.
See Table~\ref{tab:depth}.


\noindent\textbf{Depth Budget and CKKS Parameters}
\label{subsec:depth_budget}
\label{sec:pipeline:params}

Table~\ref{tab:depth} summarizes the depth accounting for both
pipelines.

\begin{table}[t]
  \centering
  \caption{Multiplicative depth accounting for both \name{} pipelines.
  Each pipeline encrypts the input into fresh depth-0 ciphertexts.}
  \label{tab:depth}
  \footnotesize
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{@{}lccp{0.30\columnwidth}@{}}
    \toprule
    \textbf{Stage} & \textbf{Depth} & \textbf{$\Sigma$}
      & \textbf{Operation} \\
    \midrule
    \multicolumn{4}{@{}l}{\textit{Pipeline 1: Vital Signs (depth 11, $N{=}32768$)}} \\
    \;\;Energy integ. & 1 & 1 & $\mathrm{Re}^2{+}\mathrm{Im}^2$ \\
    \;\;Soft attention & 1 & 2 & $E_r^2$ ($\gamma{=}2$) {\scriptsize$[\to \hat{r}]$} \\
    \;\;Phase extr. & 1 & 3 & $(|z|^2)^2{\cdot}z$, sum \\
    \;\;FIR filter & 1 & 4 & pt-ct tap accumulation \\
    \;\;Taylor arctan & 3 & 7 & $y x^2{-}y^3/3$ (3rd-order) \\
    \;\;Window + DFT & 1 & 8 & pt-ct inner product \\
    \;\;$|X|^2$ & 1 & 9 & $\mathrm{Re}^2{+}\mathrm{Im}^2$ \\
    \;\;Merge + sharp$^2$ & 1 & 10 & Merge + squaring \\
    \;\;Wt.\ freq.\ avg. & 1 & 11 & pt-ct + sum {\scriptsize$[\to \mathrm{BPM}]$} \\
    \midrule
    \multicolumn{4}{@{}l}{\textit{Pipeline 2: Dynamic Classification (depth 11, $N{=}32768$)}} \\
    \;\;Doppler DFT & 1 & 1 & BSGS block-diag matmul \\
    \;\;$|z|^2$ & 1 & 2 & $\mathrm{Re}^2{+}\mathrm{Im}^2$ \\
    \;\;Notch mask & 1 & 3 & Plaintext $\times$ cipher \\
    \;\;Soft power $\gamma{=}4$ & 2 & 5 & Two squarings \\
    \;\;Feature weighting & 1 & 6 & $p \times w$ \\
    \;\;Frame accum. & 0 & 6 & Addition only \\
    \;\;FC$_1$ + square & 2 & 8 & Matmul + $x^2$ \\
    \;\;FC$_2$ + square & 2 & 10 & Matmul + $x^2$ \\
    \;\;FC$_3$ & 1 & 11 & Matmul (final logits) \\
    \bottomrule
  \end{tabular}
\end{table}

Table~\ref{tab:depth} summarizes depth accounting.
Both pipelines use $N{=}32768$, FLEXIBLEAUTO rescaling, and
$\geq 128$-bit security without bootstrapping
(Table~\ref{tab:ckks_params}). The CKKS multiplicative depth
parameter ($L{=}14$ for vital signs, $L{=}11$ for classification)
accounts for FLEXIBLEAUTO overhead beyond the circuit depth shown in
the table. All decryptions occur on the trusted client at protocol
boundaries; every kernel processes all bins, frames, and neurons
uniformly regardless of the encrypted input
(Theorem~\ref{thm:data_oblivious}).


==> sections/5-mmFHE_updatefeb18.tex <==
\section{\name{}: System Design}
\label{sec:system_design}

We now present \name{}, a privacy-preserving pipeline that enables the cloud to perform complex radar signal processing---specifically target tracking and vital sign extraction---without decrypting the raw data. \name{} overcomes the limitations of CKKS (which lacks non-linear comparison operations) by replacing standard decision logic with differentiable, polynomial approximations that execute within a fixed multiplicative depth budget.

\subsection{High-Level Architecture}
\label{subsec:architecture}

The architecture of \name{}, illustrated in Figure~\ref{fig:arch}, consists of three stages: Client-Side Pre-processing, Cloud-Side Oblivious Processing, and Client-Side Result Recovery.

\begin{figure}[h]
    \centering
    % \includegraphics[width=\linewidth]{figures/architecture_diagram.pdf}
    \caption{The \name{} Architecture. The client captures, normalizes, and encrypts raw ADC/Range data. The cloud performs oblivious target tracking and phase extraction on encrypted data. The client decrypts and extracts vital signs from the recovered phase trace.}
    \label{fig:arch}
\end{figure}

\noindent\textbf{Key Generation.}
The client generates a CKKS key pair $(pk, sk)$ and a set of Galois keys (rotation keys). The public key $pk$ and Galois keys are sent to the cloud to enable arithmetic on ciphertexts, while the secret key $sk$ remains strictly on the client device.

\noindent\textbf{Protocol Overview.}
The \name{} protocol involves multiple encrypt--compute--decrypt stages rather than a single end-to-end encrypted pipeline. Each cloud-side primitive operates on freshly encrypted inputs and returns encrypted outputs that the client decrypts before the next stage. This staged design keeps the maximum multiplicative depth of any single encrypted computation to $L=3$ (phase extraction), well within the budget afforded by the CKKS parameter set $[60, 40, 40, 40, 40, 60]$~bits.
Crucially, all intermediate decryptions occur \emph{on the trusted client}; the cloud never observes any plaintext values.

\subsection{Client-Side Pre-processing}
\label{subsec:client_preprocessing}

To minimize the computational burden on the battery-constrained edge device, \name{} offloads the majority of the DSP chain to the cloud. The client performs only lightweight pre-processing steps that require no significant computation.

\noindent\textbf{ADC Capture \& Range-FFT.}
Commercial mmWave radars provide data either as raw ADC samples or pre-computed Range Profiles (1D-FFT). Without loss of generality, we assume the input is a sequence of complex Range Profiles $\mathbf{z}[t] \in \mathbb{C}^R$ for frames $t = 1, \ldots, F$, where $R$ is the number of range bins and $F$ is the window length.

\noindent\textbf{Clutter Removal.}
The client computes the mean range profile across the window and subtracts it from each frame: $\tilde{\mathbf{z}}[t] = \mathbf{z}[t] - \bar{\mathbf{z}}$, where $\bar{\mathbf{z}} = \frac{1}{F}\sum_{t=1}^{F}\mathbf{z}[t]$. This removes static reflections (walls, furniture) and isolates moving targets. Since this operation requires access to plaintext data, it is performed client-side before encryption.

\noindent\textbf{Normalization.}
The client normalizes the clutter-removed data such that $|\tilde{z}_r[t]| \le 1.0$ for all $r, t$, preventing scalar overflow during homomorphic squaring operations in the CKKS fixed-point representation.

\noindent\textbf{Encryption \& Packing.}
Efficiency in FHE relies on Single Instruction, Multiple Data (SIMD) packing. We pack the $R$ complex range bins from a single time frame into one ciphertext. With polynomial degree $N = 16384$, each ciphertext provides $N/2 = 8192$ complex slots, accommodating the range profile of a single frame with room for multiple receiver channels.

\subsection{Cloud-Side Oblivious Processing}
\label{subsec:cloud_processing}

The core contribution of \name{} is a set of four homomorphic primitives that replicate the functionality of standard radar algorithms (peak detection, phase tracking, and bandpass filtering) using only addition, multiplication, and plaintext-ciphertext operations. Each primitive is \emph{data-oblivious}: it processes all range bins and time frames uniformly, regardless of which bins contain targets, eliminating memory-access-pattern side channels.

\subsubsection{Primitive 1: Homomorphic Energy Integration}
\label{subsub:energy}
For each range bin $r$, the cloud computes the time-integrated energy from the encrypted range profiles:
\begin{equation}
\label{eq:energy}
    E_r = \sum_{t=1}^{F} \bigl(\mathrm{Re}(\tilde{z}_r[t])^2 + \mathrm{Im}(\tilde{z}_r[t])^2\bigr)
\end{equation}
This requires one ciphertext squaring per bin (multiplicative depth~1) followed by a rotation-and-add reduction across frames. The output is a set of $R$ encrypted energy scalars, one per range bin.

\subsubsection{Primitive 2: Homomorphic Soft-Argmax}
\label{subsub:soft_argmax}
Standard radar tracking relies on $\arg\max$ to find the range bin $r^*$ with the maximum energy---a non-linear, discontinuous operation impossible in CKKS. We replace it with a differentiable \textit{Soft-Argmax}.

The target location $\hat{r}$ is approximated as the expected value of the energy distribution raised to a sharpening power $P$:
\begin{equation}
\label{eq:soft_argmax}
    \hat{r} = \frac{\sum_{r} r \cdot E_r^P}{\sum_{r} E_r^P}
\end{equation}
As $P \to \infty$, this converges to a one-hot selector at the true peak. We use $P = 4$, implemented as two successive squarings (depth~2).

\paragraph{Normalization Protocol.}
Computing $E_r^P$ requires the energy values to be normalized to prevent overflow in the CKKS fixed-point representation. Since finding the maximum is a non-polynomial operation, we employ a client-assisted normalization step: the client decrypts the $R$ encrypted energy scalars, divides each by the maximum value, and re-encrypts the normalized profile. The cloud then applies $\mathsf{pow}(P)$ to the fresh ciphertext.
This round-trip is a fixed protocol step executed unconditionally for every window---the cloud always sends exactly $R$ encrypted scalars and receives exactly one encrypted vector in return, regardless of the energy distribution. The client is trusted and already holds the secret key, so decrypting intermediate values does not expand the attack surface. We analyze the cloud-side leakage from this interaction in Section~\ref{subsec:leakage}.

The soft-argmax also produces a \textit{soft-mask} vector $\mathbf{w}$ where $w_r = E_r^P / \sum_k E_k^P$, used by the next primitive to extract the target signal without resolving the discrete index $r^*$.

\subsubsection{Primitive 3: Homomorphic Phase Extraction}
\label{subsub:phase_extraction}
Once the soft-mask $\mathbf{w}$ is available, the cloud must extract the phase of the target's complex signal across time. In standard processing, this is a simple look-up $y[t] = z_{r^*}[t]$; in \name{}, since the cloud does not know $r^*$, we use a \textit{blind weighted extraction}.

For each frame $t$, the cloud constructs a per-bin soft mask from the encrypted range profile and applies it to extract the in-phase and quadrature components:
\begin{equation}
\label{eq:phase_iq}
    I[t] = \sum_{r=0}^{R-1} m_r[t] \cdot \mathrm{Re}(\tilde{z}_r[t]), \quad
    Q[t] = \sum_{r=0}^{R-1} m_r[t] \cdot \mathrm{Im}(\tilde{z}_r[t])
\end{equation}
where the mask $m_r[t] = \bigl(\mathrm{Re}(\tilde{z}_r[t])^2 + \mathrm{Im}(\tilde{z}_r[t])^2\bigr)^2$ is computed via two successive squarings (depth~2) followed by a ciphertext--ciphertext multiply with the original signal (depth~3). This is the deepest encrypted operation in \name{}, consuming 3 of the 4 available multiplicative levels.

The client decrypts the $(I[t], Q[t])$ pairs and computes the \textit{differential phase}:
\begin{equation}
\label{eq:diff_phase}
    \Delta\phi[t] = \angle\bigl(w[t] \cdot \overline{w[t-1]}\bigr), \quad w[t] = I[t] + jQ[t]
\end{equation}
where $\overline{(\cdot)}$ denotes complex conjugation. This differential formulation avoids the numerically unstable phase-unwrapping step ($\mathtt{np.unwrap}$) that would amplify CKKS noise over long recordings.

\subsubsection{Primitive 4: Homomorphic FIR Filtering}
\label{subsub:fir_filter}
The extracted phase trace $\Delta\phi[t]$ contains broadband noise and must be filtered to isolate the physiological bands of interest (0.1--0.5~Hz for respiration, 0.8--2.0~Hz for heart rate). We implement a Finite Impulse Response (FIR) bandpass filter in the encrypted domain.

Given the encrypted phase vector $\boldsymbol{\phi} \in \mathbb{R}^F$ (re-encrypted by the client) and plaintext filter coefficients $\mathbf{h} \in \mathbb{R}^K$ (designed via the Remez exchange algorithm), the filtered output is computed via a Toeplitz matrix--vector product:
\begin{equation}
\label{eq:toeplitz}
    \boldsymbol{\phi}_{filt} = \mathbf{T}_{\mathbf{h}} \cdot \boldsymbol{\phi}
\end{equation}
where $\mathbf{T}_{\mathbf{h}} \in \mathbb{R}^{F \times F}$ is the Toeplitz convolution matrix constructed from $\mathbf{h}$. This is implemented as a single plaintext-matrix $\times$ ciphertext-vector multiplication (depth~1), which is more efficient than the rotation-based convolution $\sum_k h_k \cdot \mathsf{Rot}(\boldsymbol{\phi}, k)$ when the FHE library provides optimized matrix--vector routines but does not expose ciphertext rotation primitives.

\subsection{Client-Side Result Recovery}
\label{subsec:result_recovery}

The client decrypts the filtered phase trace $\boldsymbol{\phi}_{filt}$ and performs spectral estimation in plaintext. A power spectral density (PSD) analysis identifies the dominant frequency peaks within the respiration band (0.1--0.5~Hz) and heart rate band (0.8--2.0~Hz), yielding the final vital sign estimates. This lightweight spectral analysis (a single FFT and peak-finding) is the only non-trivial client-side computation beyond encryption/decryption.

\subsection{Depth Budget Summary}
\label{subsec:depth_budget}

Table~\ref{tab:depth} summarizes the multiplicative depth consumed by each primitive. The CKKS parameter set $[60, 40, 40, 40, 40, 60]$~bits provides $L = 4$ multiplicative levels. Since each primitive operates on independently encrypted inputs (via the staged protocol), the maximum depth consumed in any single encrypted computation is 3 (Phase Extraction), leaving one level of headroom.

\begin{table}[h]
    \centering
    \caption{Multiplicative depth budget per primitive.}
    \label{tab:depth}
    \begin{tabular}{@{}lcc@{}}
    \toprule
    \textbf{Primitive} & \textbf{Depth} & \textbf{Key Operation} \\
    \midrule
    1. Energy Integration & 1 & $|z|^2$ (squaring) \\
    2. Soft-Argmax & 2 & $E^4$ (two squarings) \\
    3. Phase Extraction & 3 & square $\to$ square $\to$ multiply \\
    4. FIR Filter & 1 & Toeplitz matmul \\
    \midrule
    \textbf{Max single-chain depth} & \textbf{3} & (Phase Extraction) \\
    \textbf{Available depth ($L$)} & \textbf{4} & $[60,40,40,40,40,60]$ bits \\
    \bottomrule
    \end{tabular}
\end{table}

==> sections/7-implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\subsection{Software and Hardware}

We implement both \name{} pipelines in C++ using
OpenFHE~\cite{openfhe} (CPU) and FIDESlib~\cite{fideslib} (GPU)
as RNS-CKKS backends with FLEXIBLEAUTO rescaling.
Both backends use identical CKKS parameters (Table~\ref{tab:depth}).
All experiments run on a single workstation with an AMD Ryzen~9 5950X
(16C/32T), 64\,GB RAM, and an NVIDIA RTX~3090\,Ti (24\,GB, CUDA~12.9).
Client-side encryption and decryption run on the same machine for
benchmarking; in deployment they would execute on an edge device
co-located with the radar sensor.

\subsection{Datasets}

We evaluate on three public FMCW radar datasets spanning two sensing
modalities.
Table~\ref{tab:dataset_config} summarizes the radar configuration
for each dataset.

\begin{table}[t]
  \centering
  \caption{Radar and dataset configurations. All datasets are publicly
  available.}
  \label{tab:dataset_config}
  \footnotesize
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{@{}l l cccccc@{}}
    \toprule
    \textbf{Dataset} & \textbf{Task}
      & \textbf{Radar} & $f_c$ & \textbf{BW}
      & \textbf{FPS} & \textbf{Subj.} & \textbf{GT} \\
    & & & (GHz) & (GHz) & (Hz) & & \\
    \midrule
    Children~\cite{yoo2021children}
      & Vital & IWR6843 & 60 & 3.75 & 20 & 50 & BSM6501K \\
    Parralejo~\cite{parralejo2026}
      & Vital & IWR6843ISK & 60.25 & 0.48 & 10 & 110 & ECG \\
    Zenodo~\cite{seifi2024gesture}
      & Gesture & BGT60TR13C & 60.5 & 4 & 33 & 8 & Labels \\
    \bottomrule
  \end{tabular}
\end{table}

For vital signs we use
\textbf{Children}~\cite{yoo2021children} (50 pediatric subjects)
and \textbf{Parralejo}~\cite{parralejo2026} (110 subjects, lying/sitting $\times$ rest/post-exercise).
For gesture recognition we use \textbf{Zenodo 60\,GHz}~\cite{seifi2024gesture} (21{,}000 samples, 5 classes, 6 environments).

